GaitTAKE: Gait Recognition by Temporal Attention and Keypoint-guided Embedding

Gait recognition, which refers to the recognition or identification of a person based on their body shape and walking styles, derived from video data captured from a distance, is widely used in crime prevention, forensic identification, and social security. However, to the best of our knowledge, most of the existing methods use appearance, posture and temporal feautures without considering a learned temporal attention mechanism for global and local information fusion. In this paper, we propose a novel gait recognition framework, called Temporal Attention and Keypoint-guided Embedding (GaitTAKE), which effectively fuses temporal-attention-based global and local appearance feature and temporal aggregated human pose feature. Experimental results show that our proposed method achieves a new SOTA in gait recognition with rank-1 accuracy of 98.0% (normal), 97.5% (bag) and 92.2% (coat) on the CASIA-B gait dataset; 90.4% accuracy on the OU-MVLP gait dataset.

==> Tables/table1.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}
\begin{center}
\footnotesize
\caption{Rank-1 accuracy (\%) of the proposed method on CASIA-B under all views, diffeent size of training data and conditions, excluding identical-view cases. The  three walking conditions of sequences include normal  (NM),  walking  with  bag(BG) and wearing coat or jacket (CL).}\label{tab:casiab_results}
\begin{tabular}{ccccccccccccccc}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{}} & \multicolumn{1}{c|}{\multirow{2}{*}{Probe}} & \multicolumn{1}{c|}{\multirow{2}{*}{Method}} & \multicolumn{12}{c|}{Probe View} \\ 
\cline{4-15} 
\multicolumn{1}{|c|}{} &
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0$^{\circ}$}             & \multicolumn{1}{c|}{18$^{\circ}$}            & \multicolumn{1}{c|}{36$^{\circ}$}            & \multicolumn{1}{c|}{54$^{\circ}$}            & \multicolumn{1}{c|}{72$^{\circ}$}            & \multicolumn{1}{c|}{90}   & \multicolumn{1}{c|}{108$^{\circ}$}  & \multicolumn{1}{c|}{126$^{\circ}$}  & \multicolumn{1}{c|}{144$^{\circ}$}  & \multicolumn{1}{c|}{162$^{\circ}$}  & \multicolumn{1}{c|}{180$^{\circ}$}  & \multicolumn{1}{c|}{\textbf{Mean}} \\ 
\hline\hline
\multicolumn{1}{|c|}{\multirow{9}{*}{ST(24)}} &
\multicolumn{1}{c|}{\multirow{3}{*}{NM\#5-6}}    & \multicolumn{1}{c|}{Gaitset \cite{chao2019gaitset}}        & \multicolumn{1}{c|}{64.6}          & \multicolumn{1}{c|}{83.3}          & \multicolumn{1}{c|}{{90.4}}          & \multicolumn{1}{c|}{86.5}          & \multicolumn{1}{c|}{80.2}          & \multicolumn{1}{c|}{75.5} & \multicolumn{1}{c|}{80.3} & \multicolumn{1}{c|}{86.0} & \multicolumn{1}{c|}{87.1} & \multicolumn{1}{c|}{81.4} & \multicolumn{1}{c|}{59.6} & \multicolumn{1}{c|}{79.5} \\ 
\cline{3-15} 
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{}    & \multicolumn{1}{c|}{MT3D \cite{lin2020gait}}           & \multicolumn{1}{c|}{71.9}          & \multicolumn{1}{c|}{83.9}          & \multicolumn{1}{c|}{90.9}          & \multicolumn{1}{c|}{90.1}          & \multicolumn{1}{c|}{81.1}          & \multicolumn{1}{c|}{75.6} & \multicolumn{1}{c|}{82.1} & \multicolumn{1}{c|}{89.0} & \multicolumn{1}{c|}{91.1} & \multicolumn{1}{c|}{86.3} & \multicolumn{1}{c|}{69.2} & \multicolumn{1}{c|}{82.8} \\ 
\cline{3-15}
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{}    & \multicolumn{1}{c|}{GaitGL \cite{lin2020learning}}           & \multicolumn{1}{c|}{72.1}          & \multicolumn{1}{c|}{83.4}          & \multicolumn{1}{c|}{88.6}          & \multicolumn{1}{c|}{88.6}          & \multicolumn{1}{c|}{80.9}          & \multicolumn{1}{c|}{74.4} & \multicolumn{1}{c|}{82.3} & \multicolumn{1}{c|}{88.3} & \multicolumn{1}{c|}{89.5} & \multicolumn{1}{c|}{86.5} & \multicolumn{1}{c|}{69.9} & \multicolumn{1}{c|}{82.2} \\ 
\cline{3-15} 
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{}    & \multicolumn{1}{c|}{\textbf{GaitTAKE} (Ours)}       & \multicolumn{1}{c|}{\textbf{77.5}}          & \multicolumn{1}{c|}{\textbf{88.3}}          & \multicolumn{1}{c|}{\textbf{91.5}}          & \multicolumn{1}{c|}{\textbf{91.5}}          & \multicolumn{1}{c|}{\textbf{87.9}}          & \multicolumn{1}{c|}{\textbf{80.4}} & \multicolumn{1}{c|}{\textbf{87.3}} & \multicolumn{1}{c|}{\textbf{91.1}} & \multicolumn{1}{c|}{\textbf{92.5}} & \multicolumn{1}{c|}{\textbf{89.0}} & \multicolumn{1}{c|}{\textbf{74.8}} & \multicolumn{1}{c|}{\textbf{86.5}} \\ 
\cline{2-15} 
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{\multirow{3}{*}{BG\#1-2}}                       & \multicolumn{1}{c|}{Gaitset \cite{chao2019gaitset}}        & \multicolumn{1}{c|}{55.8}          & \multicolumn{1}{c|}{70.5}          & \multicolumn{1}{c|}{76.9}          & \multicolumn{1}{c|}{75.5}          & \multicolumn{1}{c|}{69.7}          & \multicolumn{1}{c|}{63.4} & \multicolumn{1}{c|}{68.0} & \multicolumn{1}{c|}{75.8} & \multicolumn{1}{c|}{76.2} & \multicolumn{1}{c|}{70.7} & \multicolumn{1}{c|}{52.5} & \multicolumn{1}{c|}{68.6} \\ 
\cline{3-15} 
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{}    & \multicolumn{1}{c|}{MT3D \cite{lin2020gait}}           & \multicolumn{1}{c|}{64.5}          & \multicolumn{1}{c|}{76.7}          & \multicolumn{1}{c|}{82.8}          & \multicolumn{1}{c|}{82.8}          & \multicolumn{1}{c|}{73.2}          & \multicolumn{1}{c|}{66.9} & \multicolumn{1}{c|}{74.0} & \multicolumn{1}{c|}{81.9} & \multicolumn{1}{c|}{84.8} & \multicolumn{1}{c|}{80.2} & \multicolumn{1}{c|}{63.0} & \multicolumn{1}{c|}{74.0} \\
\cline{3-15}
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{}    & \multicolumn{1}{c|}{GaitGL \cite{lin2020learning}}           & \multicolumn{1}{c|}{64.2}          & \multicolumn{1}{c|}{73.8}          & \multicolumn{1}{c|}{79.3}          & \multicolumn{1}{c|}{80.8}          & \multicolumn{1}{c|}{71.3}          & \multicolumn{1}{c|}{65.3} & \multicolumn{1}{c|}{72.3} & \multicolumn{1}{c|}{79.2} & \multicolumn{1}{c|}{82.5} & \multicolumn{1}{c|}{79.7} & \multicolumn{1}{c|}{60.3} & \multicolumn{1}{c|}{73.5} \\
\cline{3-15} 
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{}    & \multicolumn{1}{c|}{\textbf{GaitTAKE} (Ours)}       & \multicolumn{1}{c|}{\textbf{70.3}}          & \multicolumn{1}{c|}{\textbf{82.2}}          & \multicolumn{1}{c|}{\textbf{86.4}}          & \multicolumn{1}{c|}{\textbf{86.5}}          & \multicolumn{1}{c|}{\textbf{81.2}}          & \multicolumn{1}{c|}{\textbf{75.1}} & \multicolumn{1}{c|}{\textbf{79.8}} & \multicolumn{1}{c|}{\textbf{85.6}} & \multicolumn{1}{c|}{\textbf{87.3}} & \multicolumn{1}{c|}{\textbf{84.0}} & \multicolumn{1}{c|}{\textbf{70.5}} & \multicolumn{1}{c|}{\textbf{80.8}} \\ 
\cline{2-15} 
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{\multirow{3}{*}{CL\#1-2}}                       & \multicolumn{1}{c|}{Gaitset \cite{chao2019gaitset}}        & \multicolumn{1}{c|}{29.4} & \multicolumn{1}{c|}{43.1} & \multicolumn{1}{c|}{49.5} & \multicolumn{1}{c|}{48.7} & \multicolumn{1}{c|}{42.3} & \multicolumn{1}{c|}{40.3} & \multicolumn{1}{c|}{44.9} & \multicolumn{1}{c|}{47.4} & \multicolumn{1}{c|}{43.0} & \multicolumn{1}{c|}{35.7} & \multicolumn{1}{c|}{25.6} & \multicolumn{1}{c|}{40.9} \\ 
\cline{3-15} 
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{}    & \multicolumn{1}{c|}{MT3D \cite{lin2020gait}}           & \multicolumn{1}{c|}{46.6}          & \multicolumn{1}{c|}{{61.6}}          & \multicolumn{1}{c|}{{66.5}}          & \multicolumn{1}{c|}{63.3}          & \multicolumn{1}{c|}{57.4}          & \multicolumn{1}{c|}{52.1} & \multicolumn{1}{c|}{58.1} & \multicolumn{1}{c|}{58.9} & \multicolumn{1}{c|}{{58.5}} & \multicolumn{1}{c|}{57.4} & \multicolumn{1}{c|}{41.9} & \multicolumn{1}{c|}{56.6} \\ 
\cline{3-15} 
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{}    & \multicolumn{1}{c|}{GaitGL \cite{lin2020learning}}           & \multicolumn{1}{c|}{45.8}          & \multicolumn{1}{c|}{{59.1}}          & \multicolumn{1}{c|}{{62.7}}          & \multicolumn{1}{c|}{62.5}          & \multicolumn{1}{c|}{56.7}          & \multicolumn{1}{c|}{51.5} & \multicolumn{1}{c|}{57.6} & \multicolumn{1}{c|}{60.5} & \multicolumn{1}{c|}{{58.0}} & \multicolumn{1}{c|}{54.4} & \multicolumn{1}{c|}{37.9} & \multicolumn{1}{c|}{55.1} \\ 
\cline{3-15} 
% \multicolumn{1}{|c|}{}                       & \multicolumn{1}{c|}{Ours w/o reranking}      & \multicolumn{1}{c|}{36.9}          & \multicolumn{1}{c|}{51.8}          & \multicolumn{1}{c|}{\textbf{56.0}} & \multicolumn{1}{c|}{\textbf{57.5}} & \multicolumn{1}{c|}{\textbf{51.2}} & \multicolumn{1}{c|}{42.6} & \multicolumn{1}{c|}{50.8} & \multicolumn{1}{c|}{52.4} & \multicolumn{1}{c|}{50.7} & \multicolumn{1}{c|}{48.4} & \multicolumn{1}{c|}{34.0} & \multicolumn{1}{c|}{48.4} \\ \cline{2-14} 
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{}    & \multicolumn{1}{c|}{\textbf{GaitTAKE} (Ours)}       & \multicolumn{1}{c|}{\textbf{50.5}}          & \multicolumn{1}{c|}{\textbf{63.7}}          & \multicolumn{1}{c|}{\textbf{68.4}}          & \multicolumn{1}{c|}{\textbf{68.2}}          & \multicolumn{1}{c|}{\textbf{62.7}}          & \multicolumn{1}{c|}{\textbf{55.7}} & \multicolumn{1}{c|}{\textbf{61.7}} & \multicolumn{1}{c|}{\textbf{64.9}} & \multicolumn{1}{c|}{\textbf{63.1}} & \multicolumn{1}{c|}{\textbf{60.2}} & \multicolumn{1}{c|}{\textbf{47.6}} & \multicolumn{1}{c|}{\textbf{60.6}} \\ 
\hline\hline
\multicolumn{1}{|c|}{\multirow{9}{*}{MT(62)}} 
& \multicolumn{1}{c|}{\multirow{3}{*}{NM\#5-6}}    & \multicolumn{1}{c|}{Gaitset \cite{chao2019gaitset}}        & \multicolumn{1}{c|}{86.8}          & \multicolumn{1}{c|}{95.2}          & \multicolumn{1}{c|}{{98.0}}          & \multicolumn{1}{c|}{94.5}          & \multicolumn{1}{c|}{91.5}          & \multicolumn{1}{c|}{89.1} & \multicolumn{1}{c|}{91.1} & \multicolumn{1}{c|}{95.0} & \multicolumn{1}{c|}{97.4} & \multicolumn{1}{c|}{93.7} & \multicolumn{1}{c|}{80.2} & \multicolumn{1}{c|}{92.0} \\ 
\cline{3-15} 
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{}    & \multicolumn{1}{c|}{MT3D \cite{lin2020gait}}           & \multicolumn{1}{c|}{91.9}          & \multicolumn{1}{c|}{96.4}          & \multicolumn{1}{c|}{\textbf{98.5}}          & \multicolumn{1}{c|}{95.7}          & \multicolumn{1}{c|}{93.8}          & \multicolumn{1}{c|}{90.8} & \multicolumn{1}{c|}{93.9} & \multicolumn{1}{c|}{97.3} & \multicolumn{1}{c|}{\textbf{97.9}} & \multicolumn{1}{c|}{95.0} & \multicolumn{1}{c|}{86.8} & \multicolumn{1}{c|}{94.4} \\ 
\cline{3-15}
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{}    & \multicolumn{1}{c|}{GaitGL \cite{lin2020learning}}           & \multicolumn{1}{c|}{90.8}          & \multicolumn{1}{c|}{95.3}          & \multicolumn{1}{c|}{97.9}          & \multicolumn{1}{c|}{96.0}          & \multicolumn{1}{c|}{94.0}          & \multicolumn{1}{c|}{91.4} & \multicolumn{1}{c|}{94.7} & \multicolumn{1}{c|}{97.1} & \multicolumn{1}{c|}{97.8} & \multicolumn{1}{c|}{95.6} & \multicolumn{1}{c|}{88.0} & \multicolumn{1}{c|}{94.4} \\
\cline{3-15} 
% \multicolumn{1}{|c|}{}                       & \multicolumn{1}{c|}{Ours w/o reranking}      & \multicolumn{1}{c|}{67.2}          & \multicolumn{1}{c|}{79.5}          & \multicolumn{1}{c|}{86.4}          & \multicolumn{1}{c|}{87.2}          & \multicolumn{1}{c|}{76.4}          & \multicolumn{1}{c|}{71.5} & \multicolumn{1}{c|}{80.4} & \multicolumn{1}{c|}{87.2} & \multicolumn{1}{c|}{87.0} & \multicolumn{1}{c|}{82.4} & \multicolumn{1}{c|}{66.2} & \multicolumn{1}{c|}{79.2} \\ 
% \cline{3-15} 
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{}    & \multicolumn{1}{c|}{\textbf{GaitTAKE} (Ours)}       & \multicolumn{1}{c|}{\textbf{96.1}}          & \multicolumn{1}{c|}{\textbf{96.6}}          & \multicolumn{1}{c|}{{97.8}}          & \multicolumn{1}{c|}{\textbf{96.9}}          & \multicolumn{1}{c|}{\textbf{95.2}}          & \multicolumn{1}{c|}{\textbf{94.7}} & \multicolumn{1}{c|}{\textbf{95.7}} & \multicolumn{1}{c|}{\textbf{97.8}} & \multicolumn{1}{c|}{{97.8}} & \multicolumn{1}{c|}{\textbf{97.4}} & \multicolumn{1}{c|}{\textbf{92.6}} & \multicolumn{1}{c|}{\textbf{96.2}} \\ 
\cline{2-15} 
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{\multirow{3}{*}{BG\#1-2}}                       & \multicolumn{1}{c|}{Gaitset \cite{chao2019gaitset}}        & \multicolumn{1}{c|}{79.9}          & \multicolumn{1}{c|}{89.8}          & \multicolumn{1}{c|}{91.2}          & \multicolumn{1}{c|}{86.7}          & \multicolumn{1}{c|}{81.6}          & \multicolumn{1}{c|}{76.7} & \multicolumn{1}{c|}{81.0} & \multicolumn{1}{c|}{88.2} & \multicolumn{1}{c|}{90.3} & \multicolumn{1}{c|}{88.5} & \multicolumn{1}{c|}{73.0} & \multicolumn{1}{c|}{84.3} \\ 
\cline{3-15} 
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{}    & \multicolumn{1}{c|}{MT3D \cite{lin2020gait}}           & \multicolumn{1}{c|}{86.7}          & \multicolumn{1}{c|}{92.9}          & \multicolumn{1}{c|}{94.9}          & \multicolumn{1}{c|}{92.8}          & \multicolumn{1}{c|}{88.5}          & \multicolumn{1}{c|}{82.5} & \multicolumn{1}{c|}{87.5} & \multicolumn{1}{c|}{92.5} & \multicolumn{1}{c|}{95.3} & \multicolumn{1}{c|}{92.9} & \multicolumn{1}{c|}{81.2} & \multicolumn{1}{c|}{89.8} \\
\cline{3-15}
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{}    & \multicolumn{1}{c|}{GaitGL \cite{lin2020learning}}           & \multicolumn{1}{c|}{85.6}          & \multicolumn{1}{c|}{93.2}          & \multicolumn{1}{c|}{95.0}          & \multicolumn{1}{c|}{92.4}          & \multicolumn{1}{c|}{89.0}          & \multicolumn{1}{c|}{81.5} & \multicolumn{1}{c|}{86.6} & \multicolumn{1}{c|}{92.7} & \multicolumn{1}{c|}{95.6} & \multicolumn{1}{c|}{92.9} & \multicolumn{1}{c|}{83.1} & \multicolumn{1}{c|}{89.8} \\
\cline{3-15} 
% \multicolumn{1}{|c|}{}                       & \multicolumn{1}{c|}{Ours w/o reranking}      & \multicolumn{1}{c|}{60.3}          & \multicolumn{1}{c|}{71.2}          & \multicolumn{1}{c|}{78.1}          & \multicolumn{1}{c|}{78.0}          & \multicolumn{1}{c|}{69.0}          & \multicolumn{1}{c|}{61.2} & \multicolumn{1}{c|}{70.6} & \multicolumn{1}{c|}{77.6} & \multicolumn{1}{c|}{78.5} & \multicolumn{1}{c|}{75.7} & \multicolumn{1}{c|}{60.1} & \multicolumn{1}{c|}{70.9} \\ 
% \cline{3-15} 
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{}    & \multicolumn{1}{c|}{\textbf{GaitTAKE} (Ours)}       & \multicolumn{1}{c|}{\textbf{93.7}}          & \multicolumn{1}{c|}{\textbf{95.4}}          & \multicolumn{1}{c|}{\textbf{96.1}}          & \multicolumn{1}{c|}{\textbf{95.5}}          & \multicolumn{1}{c|}{\textbf{93.8}}          & \multicolumn{1}{c|}{\textbf{90.6}} & \multicolumn{1}{c|}{\textbf{93.5}} & \multicolumn{1}{c|}{\textbf{95.5}} & \multicolumn{1}{c|}{\textbf{96.0}} & \multicolumn{1}{c|}{\textbf{96.0}} & \multicolumn{1}{c|}{\textbf{91.3}} & \multicolumn{1}{c|}{\textbf{94.3}} \\ 
\cline{2-15} 
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{\multirow{3}{*}{CL\#1-2}}                       & \multicolumn{1}{c|}{Gaitset \cite{chao2019gaitset}}        & \multicolumn{1}{c|}{52.0} & \multicolumn{1}{c|}{66.0} & \multicolumn{1}{c|}{72.8} & \multicolumn{1}{c|}{69.3} & \multicolumn{1}{c|}{63.1} & \multicolumn{1}{c|}{61.2} & \multicolumn{1}{c|}{63.5} & \multicolumn{1}{c|}{66.5} & \multicolumn{1}{c|}{67.5} & \multicolumn{1}{c|}{66.0} & \multicolumn{1}{c|}{45.9} & \multicolumn{1}{c|}{62.5} \\ 
\cline{3-15} 
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{}    & \multicolumn{1}{c|}{MT3D \cite{lin2020gait}}           & \multicolumn{1}{c|}{67.5}          & \multicolumn{1}{c|}{{81.0}}          & \multicolumn{1}{c|}{{85.0}}          & \multicolumn{1}{c|}{80.6}          & \multicolumn{1}{c|}{75.9}          & \multicolumn{1}{c|}{69.8} & \multicolumn{1}{c|}{76.8} & \multicolumn{1}{c|}{81.0} & \multicolumn{1}{c|}{{80.8}} & \multicolumn{1}{c|}{73.8} & \multicolumn{1}{c|}{59.0} & \multicolumn{1}{c|}{75.6} \\ 
\cline{3-15}
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{}    & \multicolumn{1}{c|}{GaitGL \cite{lin2020learning}}           & \multicolumn{1}{c|}{70.2}          & \multicolumn{1}{c|}{83.6}          & \multicolumn{1}{c|}{87.3}          & \multicolumn{1}{c|}{85.2}          & \multicolumn{1}{c|}{78.5}          & \multicolumn{1}{c|}{73.1} & \multicolumn{1}{c|}{80.0} & \multicolumn{1}{c|}{85.1} & \multicolumn{1}{c|}{84.6} & \multicolumn{1}{c|}{76.9} & \multicolumn{1}{c|}{61.7} & \multicolumn{1}{c|}{78.7} \\
\cline{3-15} 
% \multicolumn{1}{|c|}{}                       & \multicolumn{1}{c|}{Ours w/o reranking}      & \multicolumn{1}{c|}{36.9}          & \multicolumn{1}{c|}{51.8}          & \multicolumn{1}{c|}{\textbf{56.0}} & \multicolumn{1}{c|}{\textbf{57.5}} & \multicolumn{1}{c|}{\textbf{51.2}} & \multicolumn{1}{c|}{42.6} & \multicolumn{1}{c|}{50.8} & \multicolumn{1}{c|}{52.4} & \multicolumn{1}{c|}{50.7} & \multicolumn{1}{c|}{48.4} & \multicolumn{1}{c|}{34.0} & \multicolumn{1}{c|}{48.4} \\ \cline{3-15} 
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{}    & \multicolumn{1}{c|}{\textbf{GaitTAKE} (Ours)}       & \multicolumn{1}{c|}{\textbf{78.7}}          & \multicolumn{1}{c|}{\textbf{90.5}}          & \multicolumn{1}{c|}{\textbf{92.5}}          & \multicolumn{1}{c|}{\textbf{89.7}}          & \multicolumn{1}{c|}{\textbf{86.6}}          & \multicolumn{1}{c|}{\textbf{82.6}} & \multicolumn{1}{c|}{\textbf{87.0}} & \multicolumn{1}{c|}{\textbf{89.4}} & \multicolumn{1}{c|}{\textbf{89.3}} & \multicolumn{1}{c|}{\textbf{87.1}} & \multicolumn{1}{c|}{\textbf{78.4}} & \multicolumn{1}{c|}{\textbf{86.5}} \\ 
\hline\hline
\multicolumn{1}{|c|}{\multirow{9}{*}{LT(74)}} 
& \multicolumn{1}{c|}{\multirow{5}{*}{NM\#5-6}}    & \multicolumn{1}{c|}{Gaitset \cite{chao2019gaitset}}        & \multicolumn{1}{c|}{90.8}          & \multicolumn{1}{c|}{97.9}          & \multicolumn{1}{c|}{\textbf{99.4}}          & \multicolumn{1}{c|}{96.9}          & \multicolumn{1}{c|}{93.6}          & \multicolumn{1}{c|}{91.7} & \multicolumn{1}{c|}{95.0} & \multicolumn{1}{c|}{97.8} & \multicolumn{1}{c|}{98.9} & \multicolumn{1}{c|}{96.8} & \multicolumn{1}{c|}{85.8} & \multicolumn{1}{c|}{95.0} \\ 
\cline{3-15} 
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{}    & \multicolumn{1}{c|}{MT3D \cite{lin2020gait}}           & \multicolumn{1}{c|}{95.7}          & \multicolumn{1}{c|}{98.2}          & \multicolumn{1}{c|}{99.0}          & \multicolumn{1}{c|}{97.5}          & \multicolumn{1}{c|}{95.1}          & \multicolumn{1}{c|}{93.9} & \multicolumn{1}{c|}{96.1} & \multicolumn{1}{c|}{98.6} & \multicolumn{1}{c|}{\textbf{99.2}} & \multicolumn{1}{c|}{98.2} & \multicolumn{1}{c|}{92.0} & \multicolumn{1}{c|}{96.7} \\ 
\cline{3-15}
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{}    & \multicolumn{1}{c|}{GaitGL \cite{lin2020learning}}           & \multicolumn{1}{c|}{94.6}          & \multicolumn{1}{c|}{97.3}          & \multicolumn{1}{c|}{{98.8}}          & \multicolumn{1}{c|}{97.1}          & \multicolumn{1}{c|}{95.8}          & \multicolumn{1}{c|}{94.3} & \multicolumn{1}{c|}{96.4} & \multicolumn{1}{c|}{98.5} & \multicolumn{1}{c|}{98.6} & \multicolumn{1}{c|}{98.2} & \multicolumn{1}{c|}{90.8} & \multicolumn{1}{c|}{96.4} \\ 
\cline{3-15} 
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{}    & \multicolumn{1}{c|}{GaitPart \cite{fan2020gaitpart}}           & \multicolumn{1}{c|}{94.1}          & \multicolumn{1}{c|}{98.6}          & \multicolumn{1}{c|}{99.3}          & \multicolumn{1}{c|}{98.5}          & \multicolumn{1}{c|}{94.0}          & \multicolumn{1}{c|}{92.3} & \multicolumn{1}{c|}{95.9} & \multicolumn{1}{c|}{98.4} & \multicolumn{1}{c|}{\textbf{99.2}} & \multicolumn{1}{c|}{97.8} & \multicolumn{1}{c|}{90.4} & \multicolumn{1}{c|}{96.2} \\ 
\cline{3-15}
% \multicolumn{1}{|c|}{}                       & \multicolumn{1}{c|}{Ours w/o reranking}      & \multicolumn{1}{c|}{67.2}          & \multicolumn{1}{c|}{79.5}          & \multicolumn{1}{c|}{86.4}          & \multicolumn{1}{c|}{87.2}          & \multicolumn{1}{c|}{76.4}          & \multicolumn{1}{c|}{71.5} & \multicolumn{1}{c|}{80.4} & \multicolumn{1}{c|}{87.2} & \multicolumn{1}{c|}{87.0} & \multicolumn{1}{c|}{82.4} & \multicolumn{1}{c|}{66.2} & \multicolumn{1}{c|}{79.2} \\ 
% \cline{3-15} 
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{}    & \multicolumn{1}{c|}{\textbf{GaitTAKE} (Ours)}        & \multicolumn{1}{c|}{\textbf{96.7}}          & \multicolumn{1}{c|}{\textbf{98.6}}          & \multicolumn{1}{c|}{{99.1}}          & \multicolumn{1}{c|}{\textbf{98.1}}          & \multicolumn{1}{c|}{\textbf{97.3}}          & \multicolumn{1}{c|}{\textbf{96.3}} & \multicolumn{1}{c|}{\textbf{98.0}} & \multicolumn{1}{c|}{\textbf{98.9}} & \multicolumn{1}{c|}{\textbf{99.2}} & \multicolumn{1}{c|}{\textbf{99.2}} & \multicolumn{1}{c|}{\textbf{96.4}} & \multicolumn{1}{c|}{\textbf{98.0}} \\
\cline{2-15} 
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{\multirow{5}{*}{BG\#1-2}}                       & \multicolumn{1}{c|}{Gaitset \cite{chao2019gaitset}}        & \multicolumn{1}{c|}{83.8}          & \multicolumn{1}{c|}{91.2}          & \multicolumn{1}{c|}{91.8}          & \multicolumn{1}{c|}{88.8}          & \multicolumn{1}{c|}{83.3}          & \multicolumn{1}{c|}{81.0} & \multicolumn{1}{c|}{84.1} & \multicolumn{1}{c|}{90.0} & \multicolumn{1}{c|}{92.2} & \multicolumn{1}{c|}{94.4} & \multicolumn{1}{c|}{79.0} & \multicolumn{1}{c|}{87.2} \\ 
\cline{3-15} 
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{}    & \multicolumn{1}{c|}{MT3D \cite{lin2020gait}}           & \multicolumn{1}{c|}{91.0}          & \multicolumn{1}{c|}{95.4}          & \multicolumn{1}{c|}{97.5}          & \multicolumn{1}{c|}{94.2}          & \multicolumn{1}{c|}{92.3}          & \multicolumn{1}{c|}{86.9} & \multicolumn{1}{c|}{91.2} & \multicolumn{1}{c|}{95.6} & \multicolumn{1}{c|}{97.3} & \multicolumn{1}{c|}{96.4} & \multicolumn{1}{c|}{86.6} & \multicolumn{1}{c|}{93.0} \\
\cline{3-15}
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{}    & \multicolumn{1}{c|}{GaitGL \cite{lin2020learning}}            & \multicolumn{1}{c|}{90.3}          & \multicolumn{1}{c|}{94.7}          & \multicolumn{1}{c|}{95.9}          & \multicolumn{1}{c|}{94.0}          & \multicolumn{1}{c|}{91.9}          & \multicolumn{1}{c|}{86.5} & \multicolumn{1}{c|}{90.5} & \multicolumn{1}{c|}{95.5} & \multicolumn{1}{c|}{97.2} & \multicolumn{1}{c|}{96.3} & \multicolumn{1}{c|}{87.1} & \multicolumn{1}{c|}{92.7} \\ 
\cline{3-15} 
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{}    & \multicolumn{1}{c|}{GaitPart \cite{fan2020gaitpart}}           & \multicolumn{1}{c|}{89.1}          & \multicolumn{1}{c|}{94.8}          & \multicolumn{1}{c|}{96.7}          & \multicolumn{1}{c|}{95.1}          & \multicolumn{1}{c|}{88.3}          & \multicolumn{1}{c|}{94.9} & \multicolumn{1}{c|}{89.0} & \multicolumn{1}{c|}{93.5} & \multicolumn{1}{c|}{96.1} & \multicolumn{1}{c|}{93.8} & \multicolumn{1}{c|}{85.8} & \multicolumn{1}{c|}{91.5} \\ 
\cline{3-15}
% \multicolumn{1}{|c|}{}                       & \multicolumn{1}{c|}{Ours w/o reranking}      & \multicolumn{1}{c|}{60.3}          & \multicolumn{1}{c|}{71.2}          & \multicolumn{1}{c|}{78.1}          & \multicolumn{1}{c|}{78.0}          & \multicolumn{1}{c|}{69.0}          & \multicolumn{1}{c|}{61.2} & \multicolumn{1}{c|}{70.6} & \multicolumn{1}{c|}{77.6} & \multicolumn{1}{c|}{78.5} & \multicolumn{1}{c|}{75.7} & \multicolumn{1}{c|}{60.1} & \multicolumn{1}{c|}{70.9} \\ 
% \cline{3-15} 
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{}    & \multicolumn{1}{c|}{\textbf{GaitTAKE} (Ours)}        & \multicolumn{1}{c|}{\textbf{96.7}}          & \multicolumn{1}{c|}{\textbf{97.0}}          & \multicolumn{1}{c|}{\textbf{97.9}}          & \multicolumn{1}{c|}{\textbf{97.6}}          & \multicolumn{1}{c|}{\textbf{97.9}}          & \multicolumn{1}{c|}{\textbf{95.7}} & \multicolumn{1}{c|}{\textbf{97.0}} & \multicolumn{1}{c|}{\textbf{98.2}} & \multicolumn{1}{c|}{\textbf{99.0}} & \multicolumn{1}{c|}{\textbf{99.0}} & \multicolumn{1}{c|}{\textbf{96.4}} & \multicolumn{1}{c|}{\textbf{97.5}} \\ 
\cline{2-15} 
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{\multirow{5}{*}{CL\#1-2}}                       & \multicolumn{1}{c|}{Gaitset \cite{chao2019gaitset}}        & \multicolumn{1}{c|}{61.4} & \multicolumn{1}{c|}{75.4} & \multicolumn{1}{c|}{80.7} & \multicolumn{1}{c|}{77.3} & \multicolumn{1}{c|}{72.1} & \multicolumn{1}{c|}{70.1} & \multicolumn{1}{c|}{71.5} & \multicolumn{1}{c|}{73.5} & \multicolumn{1}{c|}{73.5} & \multicolumn{1}{c|}{68.4} & \multicolumn{1}{c|}{50.0} & \multicolumn{1}{c|}{70.4} \\ 
\cline{3-15} 
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{}    & \multicolumn{1}{c|}{MT3D \cite{lin2020gait}}           & \multicolumn{1}{c|}{76.0}          & \multicolumn{1}{c|}{{87.6}}          & \multicolumn{1}{c|}{{89.8}}          & \multicolumn{1}{c|}{85.0}          & \multicolumn{1}{c|}{81.2}          & \multicolumn{1}{c|}{75.7} & \multicolumn{1}{c|}{81.0} & \multicolumn{1}{c|}{84.5} & \multicolumn{1}{c|}{{85.4}} & \multicolumn{1}{c|}{82.2} & \multicolumn{1}{c|}{68.1} & \multicolumn{1}{c|}{81.5} \\ 
\cline{3-15}
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{}    & \multicolumn{1}{c|}{GaitGL \cite{lin2020learning}}           & \multicolumn{1}{c|}{76.7} & \multicolumn{1}{c|}{88.3} & \multicolumn{1}{c|}{90.7} & \multicolumn{1}{c|}{86.6} & \multicolumn{1}{c|}{82.7} & \multicolumn{1}{c|}{77.6} & \multicolumn{1}{c|}{83.5} & \multicolumn{1}{c|}{86.5} & \multicolumn{1}{c|}{88.1} & \multicolumn{1}{c|}{83.2} & \multicolumn{1}{c|}{68.7} & \multicolumn{1}{c|}{83.0} \\ 
\cline{3-15} 
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{}    & \multicolumn{1}{c|}{GaitPart \cite{fan2020gaitpart}}           & \multicolumn{1}{c|}{70.7}          & \multicolumn{1}{c|}{85.5}          & \multicolumn{1}{c|}{86.9}          & \multicolumn{1}{c|}{83.3}          & \multicolumn{1}{c|}{77.1}          & \multicolumn{1}{c|}{72.5} & \multicolumn{1}{c|}{76.9} & \multicolumn{1}{c|}{82.2} & \multicolumn{1}{c|}{83.8} & \multicolumn{1}{c|}{80.2} & \multicolumn{1}{c|}{66.5} & \multicolumn{1}{c|}{78.7} \\ 
\cline{3-15}
% \multicolumn{1}{|c|}{}                       & \multicolumn{1}{c|}{Ours w/o reranking}      & \multicolumn{1}{c|}{36.9}          & \multicolumn{1}{c|}{51.8}          & \multicolumn{1}{c|}{\textbf{56.0}} & \multicolumn{1}{c|}{\textbf{57.5}} & \multicolumn{1}{c|}{\textbf{51.2}} & \multicolumn{1}{c|}{42.6} & \multicolumn{1}{c|}{50.8} & \multicolumn{1}{c|}{52.4} & \multicolumn{1}{c|}{50.7} & \multicolumn{1}{c|}{48.4} & \multicolumn{1}{c|}{34.0} & \multicolumn{1}{c|}{48.4} \\ \cline{3-15} 
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{}    & \multicolumn{1}{c|}{\textbf{GaitTAKE} (Ours)}       & \multicolumn{1}{c|}{\textbf{89.1}}          & \multicolumn{1}{c|}{\textbf{95.3}}          & \multicolumn{1}{c|}{\textbf{96.2}}          & \multicolumn{1}{c|}{\textbf{93.9}}          & \multicolumn{1}{c|}{\textbf{91.5}}          & \multicolumn{1}{c|}{\textbf{90.5}} & \multicolumn{1}{c|}{\textbf{92.5}} & \multicolumn{1}{c|}{\textbf{93.3}} & \multicolumn{1}{c|}{\textbf{93.0}} & \multicolumn{1}{c|}{\textbf{91.8}} & \multicolumn{1}{c|}{\textbf{87.0}} & \multicolumn{1}{c|}{\textbf{92.2}} \\ 
\hline
\end{tabular}
\end{center}
\end{table*}


==> Tables/table2.tex <==
\begin{table*}
\begin{center}
\footnotesize
\caption{Rank-1 accuracy (\%) of the proposed method on OUMVLP under 14 probe views excluding identical-view cases.}\label{tab:oumvlp_results}
\begin{tabular}{cccccccccccccccc}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{Method}} & \multicolumn{15}{c|}{Probe View} \\ 
\cline{2-16} 
\multicolumn{1}{|c|}{} &
\multicolumn{1}{c|}{0$^{\circ}$} & \multicolumn{1}{c|}{15$^{\circ}$} & \multicolumn{1}{c|}{30$^{\circ}$} & \multicolumn{1}{c|}{45$^{\circ}$} & \multicolumn{1}{c|}{60$^{\circ}$} & \multicolumn{1}{c|}{75$^{\circ}$} & \multicolumn{1}{c|}{90$^{\circ}$}  & \multicolumn{1}{c|}{180$^{\circ}$}  & \multicolumn{1}{c|}{195$^{\circ}$}  & \multicolumn{1}{c|}{210$^{\circ}$}  & \multicolumn{1}{c|}{225$^{\circ}$}  & \multicolumn{1}{c|}{240$^{\circ}$}  & \multicolumn{1}{c|}{255$^{\circ}$}  & \multicolumn{1}{c|}{270$^{\circ}$}  & \multicolumn{1}{c|}{\textbf{Mean}} \\ 
\hline\hline
\multicolumn{1}{|c|}{GEINet \cite{shiraga2016geinet}} & \multicolumn{1}{c|}{11.4}          & \multicolumn{1}{c|}{29.1} & \multicolumn{1}{c|}{41.5} & \multicolumn{1}{c|}{45.5}       & \multicolumn{1}{c|}{39.5} & \multicolumn{1}{c|}{41.8} & \multicolumn{1}{c|}{38.9}       & \multicolumn{1}{c|}{14.9} & \multicolumn{1}{c|}{33.1} & \multicolumn{1}{c|}{43.2}       & \multicolumn{1}{c|}{45.6} & \multicolumn{1}{c|}{39.4} & \multicolumn{1}{c|}{40.5}       & \multicolumn{1}{c|}{36.3} &  \multicolumn{1}{c|}{35.8} \\ 
\hline
\multicolumn{1}{|c|}{Gaitset \cite{chao2019gaitset}} & \multicolumn{1}{c|}{79.5}          & \multicolumn{1}{c|}{87.9} & \multicolumn{1}{c|}{89.9}       & \multicolumn{1}{c|}{90.2} & \multicolumn{1}{c|}{88.1} & \multicolumn{1}{c|}{88.7}       & \multicolumn{1}{c|}{87.8} & \multicolumn{1}{c|}{81.7} & \multicolumn{1}{c|}{86.7}       & \multicolumn{1}{c|}{89.0} & \multicolumn{1}{c|}{89.3} & \multicolumn{1}{c|}{87.2}       & \multicolumn{1}{c|}{87.8} & \multicolumn{1}{c|}{86.2} &  \multicolumn{1}{c|}{87.1} \\ 
\hline
\multicolumn{1}{|c|}{GaitPart \cite{fan2020gaitpart}} & \multicolumn{1}{c|}{82.6}          & \multicolumn{1}{c|}{88.9} & \multicolumn{1}{c|}{90.8} & \multicolumn{1}{c|}{91.0}       & \multicolumn{1}{c|}{89.7} & \multicolumn{1}{c|}{89.9} & \multicolumn{1}{c|}{89.5}       & \multicolumn{1}{c|}{85.2} & \multicolumn{1}{c|}{88.1} & \multicolumn{1}{c|}{90.0}       & \multicolumn{1}{c|}{90.1} & \multicolumn{1}{c|}{89.0} & \multicolumn{1}{c|}{89.1}       & \multicolumn{1}{c|}{88.2} &  \multicolumn{1}{c|}{88.7} \\ 
\hline
\multicolumn{1}{|c|}{GaitGL \cite{lin2020learning}} & \multicolumn{1}{c|}{84.3}          & \multicolumn{1}{c|}{89.8} & \multicolumn{1}{c|}{90.8} & \multicolumn{1}{c|}{91.0}       & \multicolumn{1}{c|}{90.5} & \multicolumn{1}{c|}{90.3} & \multicolumn{1}{c|}{89.9}       & \multicolumn{1}{c|}{88.1} & \multicolumn{1}{c|}{87.9} & \multicolumn{1}{c|}{89.6}       & \multicolumn{1}{c|}{89.8} & \multicolumn{1}{c|}{88.9} & \multicolumn{1}{c|}{88.9}       & \multicolumn{1}{c|}{88.2} &  \multicolumn{1}{c|}{89.1} \\ 
\hline
\multicolumn{1}{|c|}{\textbf{GaitTAKE} (Ours)} & \multicolumn{1}{c|}{\textbf{87.5}}       & \multicolumn{1}{c|}{\textbf{91.0}} & \multicolumn{1}{c|}{\textbf{91.5}}                 & \multicolumn{1}{c|}{\textbf{91.8}} & \multicolumn{1}{c|}{\textbf{91.4}}                 & \multicolumn{1}{c|}{\textbf{91.1}} & \multicolumn{1}{c|}{\textbf{90.8}}                 & \multicolumn{1}{c|}{\textbf{90.2}} & \multicolumn{1}{c|}{\textbf{89.7}}                 & \multicolumn{1}{c|}{\textbf{90.5}} & \multicolumn{1}{c|}{\textbf{90.7}}                 & \multicolumn{1}{c|}{\textbf{90.3}} & \multicolumn{1}{c|}{\textbf{90.0}}                 & \multicolumn{1}{c|}{\textbf{89.5}} &  \multicolumn{1}{c|}{\textbf{90.4}} \\ 

\hline

\end{tabular}
\end{center}
\end{table*}

==> Tables/table2_old.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% \begin{table*}[]
% \small
% \begin{center}
% \begin{tabular}{|c|c|c|c|c|c|}
% \hline
% \multirow{2}{*}{Probe} & \multicolumn{5}{c|}{gallery All 14 views}     \\ \cline{2-6} 
%                       & GEINet \cite{shiraga2016geinet} & GaitSet \cite{chao2019gaitset} & GaitPart \cite{fan2020gaitpart} & GaitGL \cite{lin2020learning}  & GaitTAKE (Ours) \\ \hline
% 0                      & 11.4   & 79.5    & 82.6     & 84.3     & \textbf{87.5}   \\ \hline
% 15                     & 29.1   & 87.9    & 88.9     & 89.8     & \textbf{91.0}   \\ \hline
% 30                     & 41.5   & 89.9    & 90.8     & 90.8     & \textbf{91.5}   \\ \hline
% 45                     & 45.5   & 90.2    & 91.0     & 91.0     & \textbf{91.8}   \\ \hline
% 60                     & 39.5   & 88.1    & 89.7     & 90.5     & \textbf{91.4}   \\ \hline
% 75                     & 41.8   & 88.7    & 89.9     & 90.3     & \textbf{91.1}   \\ \hline
% 90                     & 38.9   & 87.8    & 89.5     & 89.9     & \textbf{90.8}   \\ \hline
% 180                    & 14.9   & 81.7    & 85.2     & 88.1     & \textbf{90.2}   \\ \hline
% 195                    & 33.1   & 86.7    & 88.1     & 87.9     & \textbf{89.7}   \\ \hline
% 210                    & 43.2   & 89.0    & 90.0     & 89.6     & \textbf{90.5}   \\ \hline
% 225                    & 45.6   & 89.3    & 90.1     & 89.8     & \textbf{90.7}   \\ \hline
% 240                    & 39.4   & 87.2    & 89.0     & 88.9     & \textbf{90.3}   \\ \hline
% 255                    & 40.5   & 87.8    & 89.1     & 88.9     & \textbf{90.0}   \\ \hline
% 270                    & 36.3   & 86.2    & 88.2     & 88.2     & \textbf{89.5}   \\ \hline
% mean                   & 35.8   & 87.1    & 88.7     & 89.1     & \textbf{90.4}   \\ \hline
% \end{tabular}
% \end{center}
% \caption{Rank-1 accuracy (\%) of the proposed method on OUMVLP under 14 probe views excluding identical-view cases.}\label{tab:oumvlp_results}
% \end{table*}


==> Tables/table3.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}
\begin{center}
\small
\caption{The ablation study of the proposed method on CASIA-B dataset in LT setting.}\label{tab:casiab_ablation}

\begin{tabular}{cccccccccccccc}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{Probe}} & \multicolumn{1}{c|}{\multirow{2}{*}{Method}} & \multicolumn{12}{c|}{Probe View} \\ 
\cline{3-14} 
\multicolumn{1}{|c|}{}                       & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0$^{\circ}$}             & \multicolumn{1}{c|}{18$^{\circ}$}            & \multicolumn{1}{c|}{36$^{\circ}$}            & \multicolumn{1}{c|}{54$^{\circ}$}            & \multicolumn{1}{c|}{72$^{\circ}$}            & \multicolumn{1}{c|}{90}   & \multicolumn{1}{c|}{108$^{\circ}$}  & \multicolumn{1}{c|}{126$^{\circ}$}  & \multicolumn{1}{c|}{144$^{\circ}$}  & \multicolumn{1}{c|}{162$^{\circ}$}  & \multicolumn{1}{c|}{180$^{\circ}$}  & \multicolumn{1}{c|}{\textbf{Mean}} \\ 
\hline\hline
\multicolumn{1}{|c|}{\multirow{3}{*}{NM\#5-6}}    & \multicolumn{1}{c|}{TP}        & \multicolumn{1}{c|}{94.6}          & \multicolumn{1}{c|}{97.3}          & \multicolumn{1}{c|}{{98.8}}          & \multicolumn{1}{c|}{97.1}          & \multicolumn{1}{c|}{95.8}          & \multicolumn{1}{c|}{94.3} & \multicolumn{1}{c|}{96.4} & \multicolumn{1}{c|}{98.5} & \multicolumn{1}{c|}{98.6} & \multicolumn{1}{c|}{98.2} & \multicolumn{1}{c|}{90.8} & \multicolumn{1}{c|}{96.4} \\ 
\cline{2-14} 
\multicolumn{1}{|c|}{}    & \multicolumn{1}{c|}{TA}           & \multicolumn{1}{c|}{{95.9}}          & \multicolumn{1}{c|}{{98.4}}          & \multicolumn{1}{c|}{\textbf{99.1}}          & \multicolumn{1}{c|}{\textbf{98.7}}          & \multicolumn{1}{c|}{\textbf{98.7}}          & \multicolumn{1}{c|}{\textbf{97.4}} & \multicolumn{1}{c|}{\textbf{98.6}} & \multicolumn{1}{c|}{\textbf{99.5}} & \multicolumn{1}{c|}{\textbf{99.4}} & \multicolumn{1}{c|}{{98.6}} & \multicolumn{1}{c|}{{96.0}} & \multicolumn{1}{c|}{\textbf{98.2}} \\ 
\cline{2-14} 
\multicolumn{1}{|c|}{}                       & \multicolumn{1}{c|}{TA+KE}       & \multicolumn{1}{c|}{\textbf{96.7}}          & \multicolumn{1}{c|}{\textbf{98.6}}          & \multicolumn{1}{c|}{\textbf{99.1}}          & \multicolumn{1}{c|}{{98.1}}          & \multicolumn{1}{c|}{{97.3}}          & \multicolumn{1}{c|}{{96.3}} & \multicolumn{1}{c|}{{98.0}} & \multicolumn{1}{c|}{{98.9}} & \multicolumn{1}{c|}{{99.2}} & \multicolumn{1}{c|}{\textbf{99.2}} & \multicolumn{1}{c|}{\textbf{96.4}} & \multicolumn{1}{c|}{{98.0}} \\ 
\hline\hline
\multicolumn{1}{|c|}{\multirow{3}{*}{BG\#1-2}}                       & \multicolumn{1}{c|}{TP}        & \multicolumn{1}{c|}{90.3}          & \multicolumn{1}{c|}{94.7}          & \multicolumn{1}{c|}{95.9}          & \multicolumn{1}{c|}{94.0}          & \multicolumn{1}{c|}{91.9}          & \multicolumn{1}{c|}{86.5} & \multicolumn{1}{c|}{90.5} & \multicolumn{1}{c|}{95.5} & \multicolumn{1}{c|}{97.2} & \multicolumn{1}{c|}{96.3} & \multicolumn{1}{c|}{87.1} & \multicolumn{1}{c|}{92.7} \\ 
\cline{2-14} 
\multicolumn{1}{|c|}{}    & \multicolumn{1}{c|}{TA}           & \multicolumn{1}{c|}{{95.2}}          & \multicolumn{1}{c|}{{96.5}}          & \multicolumn{1}{c|}{\textbf{98.5}}          & \multicolumn{1}{c|}{\textbf{98.9}}          & \multicolumn{1}{c|}{{96.9}}          & \multicolumn{1}{c|}{{93.0}} & \multicolumn{1}{c|}{{94.5}} & \multicolumn{1}{c|}{{97.1}} & \multicolumn{1}{c|}{{98.6}} & \multicolumn{1}{c|}{{98.3}} & \multicolumn{1}{c|}{{95.0}} & \multicolumn{1}{c|}{{96.6}} \\ 
\cline{2-14} 
\multicolumn{1}{|c|}{}                       & \multicolumn{1}{c|}{TA+KE}       & \multicolumn{1}{c|}{\textbf{96.7}}          & \multicolumn{1}{c|}{\textbf{97.0}}          & \multicolumn{1}{c|}{{97.9}}          & \multicolumn{1}{c|}{{97.6}}          & \multicolumn{1}{c|}{\textbf{97.9}}          & \multicolumn{1}{c|}{\textbf{95.7}} & \multicolumn{1}{c|}{\textbf{97.0}} & \multicolumn{1}{c|}{\textbf{98.2}} & \multicolumn{1}{c|}{\textbf{99.0}} & \multicolumn{1}{c|}{\textbf{99.0}} & \multicolumn{1}{c|}{\textbf{96.4}} & \multicolumn{1}{c|}{\textbf{97.5}} \\ 
\hline\hline
\multicolumn{1}{|c|}{\multirow{3}{*}{CL\#1-2}}                       & \multicolumn{1}{c|}{TP}        & \multicolumn{1}{c|}{76.7} & \multicolumn{1}{c|}{88.3} & \multicolumn{1}{c|}{90.7} & \multicolumn{1}{c|}{86.6} & \multicolumn{1}{c|}{82.7} & \multicolumn{1}{c|}{77.6} & \multicolumn{1}{c|}{83.5} & \multicolumn{1}{c|}{86.5} & \multicolumn{1}{c|}{88.1} & \multicolumn{1}{c|}{83.2} & \multicolumn{1}{c|}{68.7} & \multicolumn{1}{c|}{83.0} \\ 
\cline{2-14} 
\multicolumn{1}{|c|}{}    & \multicolumn{1}{c|}{TA}          & \multicolumn{1}{c|}{{76.0}}          & \multicolumn{1}{c|}{84.5}          & \multicolumn{1}{c|}{84.0}          & \multicolumn{1}{c|}{{85.1}}          & \multicolumn{1}{c|}{{85.1}}          & \multicolumn{1}{c|}{{83.8}} & \multicolumn{1}{c|}{{85.0}} & \multicolumn{1}{c|}{{87.0}} & \multicolumn{1}{c|}{85.1} & \multicolumn{1}{c|}{{84.3}} & \multicolumn{1}{c|}{{76.0}} & \multicolumn{1}{c|}{{83.3}} \\ 
\cline{2-14} 
\multicolumn{1}{|c|}{}                       & \multicolumn{1}{c|}{TA+KE}       & \multicolumn{1}{c|}{\textbf{89.1}}          & \multicolumn{1}{c|}{\textbf{95.3}}          & \multicolumn{1}{c|}{\textbf{96.2}}          & \multicolumn{1}{c|}{\textbf{93.9}}          & \multicolumn{1}{c|}{\textbf{91.5}}          & \multicolumn{1}{c|}{\textbf{90.5}} & \multicolumn{1}{c|}{\textbf{92.5}} & \multicolumn{1}{c|}{\textbf{93.3}} & \multicolumn{1}{c|}{\textbf{93.0}} & \multicolumn{1}{c|}{\textbf{91.8}} & \multicolumn{1}{c|}{\textbf{87.0}} & \multicolumn{1}{c|}{\textbf{92.2}} \\ 
\hline
\end{tabular}
\end{center}
\end{table*}

==> Tables/table3_clean.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}
\begin{center}
\small

\begin{tabular}{cccccccccccccc}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{Probe}} & \multicolumn{1}{c|}{\multirow{2}{*}{Method}} & \multicolumn{12}{c|}{Probe View} \\ 
\cline{3-14} 
\multicolumn{1}{|c|}{}                       & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c}{0$^{\circ}$}             & \multicolumn{1}{c}{18$^{\circ}$}            & \multicolumn{1}{c}{36$^{\circ}$}            & \multicolumn{1}{c}{54$^{\circ}$}            & \multicolumn{1}{c}{72$^{\circ}$}            & \multicolumn{1}{c}{90}   & \multicolumn{1}{c}{108$^{\circ}$}  & \multicolumn{1}{c}{126$^{\circ}$}  & \multicolumn{1}{c}{144$^{\circ}$}  & \multicolumn{1}{c}{162$^{\circ}$}  & \multicolumn{1}{c}{180$^{\circ}$}  & \multicolumn{1}{|c|}{\textbf{Mean}} \\ 
\hline\hline
\multicolumn{1}{|c|}{\multirow{3}{*}{NM\#5-6}}    & \multicolumn{1}{c|}{TP}        & \multicolumn{1}{c}{94.6}          & \multicolumn{1}{c}{97.3}          & \multicolumn{1}{c}{{98.8}}          & \multicolumn{1}{c}{97.1}          & \multicolumn{1}{c}{95.8}          & \multicolumn{1}{c}{94.3} & \multicolumn{1}{c}{96.4} & \multicolumn{1}{c}{98.5} & \multicolumn{1}{c}{98.6} & \multicolumn{1}{c}{98.2} & \multicolumn{1}{c}{90.8} & \multicolumn{1}{|c|}{96.4} \\ 
% \cline{2-14} 
\multicolumn{1}{|c|}{}    & \multicolumn{1}{c|}{TA}           & \multicolumn{1}{c}{{95.9}}          & \multicolumn{1}{c}{{98.4}}          & \multicolumn{1}{c}{\textbf{99.1}}          & \multicolumn{1}{c}{\textbf{98.7}}          & \multicolumn{1}{c}{\textbf{98.7}}          & \multicolumn{1}{c}{\textbf{97.4}} & \multicolumn{1}{c}{\textbf{98.6}} & \multicolumn{1}{c}{\textbf{99.5}} & \multicolumn{1}{c}{\textbf{99.4}} & \multicolumn{1}{c}{{98.6}} & \multicolumn{1}{c}{{96.0}} & \multicolumn{1}{|c|}{\textbf{98.2}} \\ 

% % \cline{2-14} 
% \multicolumn{1}{|c|}{}    & \multicolumn{1}{c|}{TP (avg)+KE}           & \multicolumn{1}{c}{{85.8}}          & \multicolumn{1}{c}{{93.8}}          & \multicolumn{1}{c}{96.0}          & \multicolumn{1}{c}{94.8}          & \multicolumn{1}{c}{91.8}          & \multicolumn{1}{c}{91.5} & \multicolumn{1}{c}{92.7} & \multicolumn{1}{c}{94.8} & \multicolumn{1}{c}{95.9} & \multicolumn{1}{c}{{94.2}} & \multicolumn{1}{c}{{85.8}} & \multicolumn{1}{|c|}{92.5} \\ 

% \cline{2-14} 
\multicolumn{1}{|c|}{}    & \multicolumn{1}{c|}{TP+KE}           & \multicolumn{1}{c}{{95.6}}          & \multicolumn{1}{c}{{97.0}}          & \multicolumn{1}{c}{97.9}          & \multicolumn{1}{c}{97.6}          & \multicolumn{1}{c}{96.8}          & \multicolumn{1}{c}{96.4} & \multicolumn{1}{c}{97.0} & \multicolumn{1}{c}{97.5} & \multicolumn{1}{c}{98.0} & \multicolumn{1}{c}{{97.9}} & \multicolumn{1}{c}{{94.4}} & \multicolumn{1}{|c|}{96.9} \\ 

% % \cline{2-14} 
% \multicolumn{1}{|c|}{}    & \multicolumn{1}{c|}{GaitGL+KE}           & \multicolumn{1}{c}{{96.1}}          & \multicolumn{1}{c}{{97.7}}          & \multicolumn{1}{c}{99.4}          & \multicolumn{1}{c}{98.7}          & \multicolumn{1}{c}{98.9}          & \multicolumn{1}{c}{98.0} & \multicolumn{1}{c}{98.3} & \multicolumn{1}{c}{99.3} & \multicolumn{1}{c}{99.3} & \multicolumn{1}{c}{{98.6}} & \multicolumn{1}{c}{{95.2}} & \multicolumn{1}{|c|}{98.1} \\ 

% \cline{2-14} 
\multicolumn{1}{|c|}{}                       & \multicolumn{1}{c|}{TA+KE}       & \multicolumn{1}{c}{\textbf{96.7}}          & \multicolumn{1}{c}{\textbf{98.6}}          & \multicolumn{1}{c}{\textbf{99.1}}          & \multicolumn{1}{c}{{98.1}}          & \multicolumn{1}{c}{{97.3}}          & \multicolumn{1}{c}{{96.3}} & \multicolumn{1}{c}{{98.0}} & \multicolumn{1}{c}{{98.9}} & \multicolumn{1}{c}{{99.2}} & \multicolumn{1}{c}{\textbf{99.2}} & \multicolumn{1}{c}{\textbf{96.4}} & \multicolumn{1}{|c|}{{98.0}} \\ 
\hline\hline
\multicolumn{1}{|c|}{\multirow{3}{*}{BG\#1-2}}                       & \multicolumn{1}{c|}{TP}        & \multicolumn{1}{c}{90.3}          & \multicolumn{1}{c}{94.7}          & \multicolumn{1}{c}{95.9}          & \multicolumn{1}{c}{94.0}          & \multicolumn{1}{c}{91.9}          & \multicolumn{1}{c}{86.5} & \multicolumn{1}{c}{90.5} & \multicolumn{1}{c}{95.5} & \multicolumn{1}{c}{97.2} & \multicolumn{1}{c}{96.3} & \multicolumn{1}{c}{87.1} & \multicolumn{1}{|c|}{92.7} \\ 
% \cline{2-14} 
\multicolumn{1}{|c|}{}    & \multicolumn{1}{c|}{TA}           & \multicolumn{1}{c}{{95.2}}          & \multicolumn{1}{c}{{96.5}}          & \multicolumn{1}{c}{\textbf{98.5}}          & \multicolumn{1}{c}{\textbf{98.9}}          & \multicolumn{1}{c}{{96.9}}          & \multicolumn{1}{c}{{93.0}} & \multicolumn{1}{c}{{94.5}} & \multicolumn{1}{c}{{97.1}} & \multicolumn{1}{c}{{98.6}} & \multicolumn{1}{c}{{98.3}} & \multicolumn{1}{c}{{95.0}} & \multicolumn{1}{|c|}{{96.6}} \\ 

% % \cline{2-14} 
% \multicolumn{1}{|c|}{}    & \multicolumn{1}{c|}{TP (avg)+KE}           & \multicolumn{1}{c}{{81.0}}          & \multicolumn{1}{c}{{87.9}}          & \multicolumn{1}{c}{90.1}          & \multicolumn{1}{c}{90.1}          & \multicolumn{1}{c}{88.8}          & \multicolumn{1}{c}{85.8} & \multicolumn{1}{c}{88.6} & \multicolumn{1}{c}{90.3} & \multicolumn{1}{c}{92.0} & \multicolumn{1}{c}{{91.1}} & \multicolumn{1}{c}{{79.4}} & \multicolumn{1}{|c|}{87.7} \\ 

% \cline{2-14} 
\multicolumn{1}{|c|}{}    & \multicolumn{1}{c|}{TP+KE}           & \multicolumn{1}{c}{{94.6}}          & \multicolumn{1}{c}{{94.2}}          & \multicolumn{1}{c}{95.2}          & \multicolumn{1}{c}{95.0}          & \multicolumn{1}{c}{93.9}          & \multicolumn{1}{c}{92.4} & \multicolumn{1}{c}{94.6} & \multicolumn{1}{c}{95.3} & \multicolumn{1}{c}{96.1} & \multicolumn{1}{c}{{95.6}} & \multicolumn{1}{c}{{92.4}} & \multicolumn{1}{|c|}{94.5} \\ 

% % \cline{2-14} 
% \multicolumn{1}{|c|}{}    & \multicolumn{1}{c|}{GaitGL+KE}           & \multicolumn{1}{c}{{94.3}}          & \multicolumn{1}{c}{{95.5}}          & \multicolumn{1}{c}{97.8}          & \multicolumn{1}{c}{98.6}          & \multicolumn{1}{c}{96.8}          & \multicolumn{1}{c}{94.3} & \multicolumn{1}{c}{95.8} & \multicolumn{1}{c}{97.2} & \multicolumn{1}{c}{97.8} & \multicolumn{1}{c}{{97.9}} & \multicolumn{1}{c}{{93.3}} & \multicolumn{1}{|c|}{96.3} \\ 


% \cline{2-14} 
\multicolumn{1}{|c|}{}                       & \multicolumn{1}{c|}{TA+KE}       & \multicolumn{1}{c}{\textbf{96.7}}          & \multicolumn{1}{c}{\textbf{97.0}}          & \multicolumn{1}{c}{{97.9}}          & \multicolumn{1}{c}{{97.6}}          & \multicolumn{1}{c}{\textbf{97.9}}          & \multicolumn{1}{c}{\textbf{95.7}} & \multicolumn{1}{c}{\textbf{97.0}} & \multicolumn{1}{c}{\textbf{98.2}} & \multicolumn{1}{c}{\textbf{99.0}} & \multicolumn{1}{c}{\textbf{99.0}} & \multicolumn{1}{c}{\textbf{96.4}} & \multicolumn{1}{|c|}{\textbf{97.5}} \\ 
\hline\hline
\multicolumn{1}{|c|}{\multirow{3}{*}{CL\#1-2}}                       & \multicolumn{1}{c|}{TP}        & \multicolumn{1}{c}{76.7} & \multicolumn{1}{c}{88.3} & \multicolumn{1}{c}{90.7} & \multicolumn{1}{c}{86.6} & \multicolumn{1}{c}{82.7} & \multicolumn{1}{c}{77.6} & \multicolumn{1}{c}{83.5} & \multicolumn{1}{c}{86.5} & \multicolumn{1}{c}{88.1} & \multicolumn{1}{c}{83.2} & \multicolumn{1}{c}{68.7} & \multicolumn{1}{|c|}{83.0} \\ 
% \cline{2-14} 
\multicolumn{1}{|c|}{}    & \multicolumn{1}{c|}{TA}          & \multicolumn{1}{c}{{76.0}}          & \multicolumn{1}{c}{84.5}          & \multicolumn{1}{c}{84.0}          & \multicolumn{1}{c}{{85.1}}          & \multicolumn{1}{c}{{85.1}}          & \multicolumn{1}{c}{{83.8}} & \multicolumn{1}{c}{{85.0}} & \multicolumn{1}{c}{{87.0}} & \multicolumn{1}{c}{85.1} & \multicolumn{1}{c}{{84.3}} & \multicolumn{1}{c}{{76.0}} & \multicolumn{1}{|c|}{{83.3}} \\ 

% % \cline{2-14} 
% \multicolumn{1}{|c|}{}    & \multicolumn{1}{c|}{TP (avg)+KE}           & \multicolumn{1}{c}{{66.1}}          & \multicolumn{1}{c}{{79.0}}          & \multicolumn{1}{c}{83.1}          & \multicolumn{1}{c}{82.0}          & \multicolumn{1}{c}{81.7}          & \multicolumn{1}{c}{77.5} & \multicolumn{1}{c}{78.8} & \multicolumn{1}{c}{80.3} & \multicolumn{1}{c}{76.2} & \multicolumn{1}{c}{{77.1}} & \multicolumn{1}{c}{{58.1}} & \multicolumn{1}{|c|}{76.4} \\ 

% \cline{2-14} 
\multicolumn{1}{|c|}{}    & \multicolumn{1}{c|}{TP+KE}           & \multicolumn{1}{c}{{84.6}}          & \multicolumn{1}{c}{{90.7}}          & \multicolumn{1}{c}{91.6}          & \multicolumn{1}{c}{89.7}          & \multicolumn{1}{c}{86.5}          & \multicolumn{1}{c}{84.1} & \multicolumn{1}{c}{87.9} & \multicolumn{1}{c}{88.8} & \multicolumn{1}{c}{89.9} & \multicolumn{1}{c}{{86.7}} & \multicolumn{1}{c}{{80.0}} & \multicolumn{1}{|c|}{87.3} \\ 

% % \cline{2-14} 
% \multicolumn{1}{|c|}{}    & \multicolumn{1}{c|}{GaitGL+KE}           & \multicolumn{1}{c}{{78.5}}          & \multicolumn{1}{c}{{86.8}}          & \multicolumn{1}{c}{85.6}          & \multicolumn{1}{c}{85.1}          & \multicolumn{1}{c}{84.9}          & \multicolumn{1}{c}{83.7} & \multicolumn{1}{c}{87.3} & \multicolumn{1}{c}{88.0} & \multicolumn{1}{c}{88.0} & \multicolumn{1}{c}{{86.5}} & \multicolumn{1}{c}{{76.4}} & \multicolumn{1}{|c|}{84.6} \\ 

% \cline{2-14} 
\multicolumn{1}{|c|}{}                       & \multicolumn{1}{c|}{TA+KE}       & \multicolumn{1}{c}{\textbf{89.1}}          & \multicolumn{1}{c}{\textbf{95.3}}          & \multicolumn{1}{c}{\textbf{96.2}}          & \multicolumn{1}{c}{\textbf{93.9}}          & \multicolumn{1}{c}{\textbf{91.5}}          & \multicolumn{1}{c}{\textbf{90.5}} & \multicolumn{1}{c}{\textbf{92.5}} & \multicolumn{1}{c}{\textbf{93.3}} & \multicolumn{1}{c}{\textbf{93.0}} & \multicolumn{1}{c}{\textbf{91.8}} & \multicolumn{1}{c}{\textbf{87.0}} & \multicolumn{1}{|c|}{\textbf{92.2}} \\ 
\hline
\end{tabular}
\vspace{1em}
\caption{The ablation study of the proposed method on CASIA-B dataset in LT setting.}\label{tab:casiab_ablation}
\end{center}
\end{table*}

==> Tables/table4.tex <==
\begin{table}[h]
% \small
\begin{center}
\begin{tabular}{c|c c c c}
\hline 
 & AP & AP50 & AP75  \\
\hline 
Keypoint-RCNN & 91.7  & 98.6 & 97.4  \\
\hline 
\end{tabular}
\end{center}
%\vspace{-1em}
\caption{The performance for keypoints R-CNN  on CASIA-B.}
\label{tab:res_key}
\end{table}
% \vspace{-1em}
